Quantum Denoising Diffusion Models

In recent years, machine learning models like DALL-E, Craiyon, and Stable Diffusion have gained significant attention for their ability to generate high-resolution images from concise descriptions. Concurrently, quantum computing is showing promising advances, especially with quantum machine learning which capitalizes on quantum mechanics to meet the increasing computational requirements of traditional machine learning algorithms. This paper explores the integration of quantum machine learning and variational quantum circuits to augment the efficacy of diffusion-based image generation models. Specifically, we address two challenges of classical diffusion models: their low sampling speed and the extensive parameter requirements. We introduce two quantum diffusion models and benchmark their capabilities against their classical counterparts using MNIST digits, Fashion MNIST, and CIFAR-10. Our models surpass the classical models with similar parameter counts in terms of performance metrics FID, SSIM, and PSNR. Moreover, we introduce a consistency model unitary single sampling architecture that combines the diffusion procedure into a single step, enabling a fast one-step image generation.

==> images/pictures/strongly.tex <==
\begin{figure*}[bt]
    \centering
    \begin{quantikz}[transparent, row sep={0.8cm,between origins}]
    \lstick{$q_0$}   & \gate{Rot} & \ctrl{0} & \qw & \qw & \targ{}\vqw{0}   & \qw \slice{} & \gate{Rot} & \ctrl{0} & \qw & \targ{}\vqw{0} & \qw & \qw     & \qw \slice{}  & \gate{Rot}  \qw & \ctrl{0} & \targ{}\vqw{0} & \qw & \qw & \qw                                              \\
    \lstick{$q_1$}   & \gate{Rot} & \targ{}\vqw{-1} & \ctrl{0} & \qw & \qw  & \qw          & \gate{Rot} & \qw & \ctrl{0} & \qw & \targ{}\vqw{0} & \qw     & \qw           & \gate{Rot}  \qw & \qw & \ctrl{-1} & \targ{}\vqw{0} & \qw & \qw                                             \\
    \lstick{$q_2$}   & \gate{Rot} & \qw & \targ{}\vqw{-1} & \ctrl{0} & \qw  & \qw          & \gate{Rot} & \targ{}\vqw{-2} & \qw & \ctrl{-2} & \qw & \qw   & \qw           & \gate{Rot}  \qw & \qw & \qw & \ctrl{-1} & \targ{}\vqw{0} & \qw                                             \\
    \lstick{$q_3$}   & \gate{Rot} & \qw & \qw & \targ{}\vqw{-1} & \ctrl{-3} & \qw          & \gate{Rot} & \qw & \targ{}\vqw{-2} & \qw & \ctrl{-2}  & \qw  & \qw           & \gate{Rot}  \qw & \targ{}\vqw{-3} & \qw & \qw & \ctrl{-1} & \qw
\end{quantikz}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure*}



==> images/pictures/twoloc.tex <==
\begin{quantikz}[transparent, row sep={0.8cm,between origins}]
    \lstick{$q_0$}   & \gate{Rot} & \ctrl{0} & \ctrl{0} & \ctrl{0} & \qw & \qw & \qw & \qw                       & \qw \slice{} & \gate{Rot} & \ctrl{0} & \ctrl{0} & \ctrl{0} & \qw & \qw & \qw & \qw                           \\
    \lstick{$q_1$}   & \gate{Rot} & \targ{}\vqw{-1} & \qw & \qw & \ctrl{0} & \ctrl{0} & \qw & \qw                & \qw           & \gate{Rot} & \targ{}\vqw{-1} & \qw & \qw & \ctrl{0} & \ctrl{0} & \qw & \qw                   \\
    \lstick{$q_2$}   & \gate{Rot} & \qw & \targ{}\vqw{-2} & \qw & \targ{}\vqw{-1} & \qw & \ctrl{0} & \qw         & \qw           & \gate{Rot} & \qw & \targ{}\vqw{-2} & \qw & \targ{}\vqw{-1} & \qw & \ctrl{0} & \qw            \\
    \lstick{$q_3$}   & \gate{Rot} & \qw & \qw & \targ{}\vqw{-3} & \qw & \targ{}\vqw{-2} & \targ{}\vqw{-1} & \qw  & \qw           & \gate{Rot} & \qw & \qw & \targ{}\vqw{-3} & \qw & \targ{}\vqw{-2} & \targ{}\vqw{-1} & \qw 
\end{quantikz}


==> images/results/eval/MNISTBIG/time.tex <==
\begin{tabular}{lr}
    \toprule
    Model Name                     & Time per Epoch (s) \\
    \midrule
    U-Net d3 s2                    & 1.000000           \\
    U-Net d2 s3                    & 1.011236           \\
    QDense d30                     & 5.022472           \\
    QDense d60                     & 10.292135          \\
    Q-U-Net d3 s2 l9               & 217.685393         \\
    Q-U-Net d3 s2 d19              & 283.191011         \\
    \bottomrule
\end{tabular}


==> images/results/eval/fashion/time.tex <==
\begin{tabular}{lr}
        \toprule
        Model         & Sampling time (s) \\
        \midrule
        UNet d3s1     & 1.00              \\
        UNet d3s2     & 1.07              \\
        QDense 60     & 106.75            \\
        QDense 121    & 221.08            \\
        QUNet d3s2d8  & 4023.41           \\
        QUNet d3s2d12 & 4153.33           \\
        QUNet d3s4d8  & 4474.04           \\
        QUNet d3s4d12 & 4867.65           \\
        \bottomrule
\end{tabular}

